Multi-mode Cavity Centric Architectures for Quantum Simulation

Near-term quantum computing technologies grapple with huge complexity overheads, hindering their ability to induce algorithms, necessitating engineering and scientific innovations. One class of problems of interest is Quantum Simulation, whereby quantum systems are simulated using a quantum computer. However, current devices are yet to surpass classical tensor network techniques. For problems of interest, where classical simulation techniques fail, large degrees of entanglement are required. Another challenge of implementing quantum simulation problems is that qubits sit idle whilst alternating simulation terms are implemented, exposing the system to decoherence. In the near term, 2D planar superconducting lattices of circuit-QED elements such as the transmon continue to draw substantial attention, but they are hindered by their nearest neighbor topology and relatively short lifespan, two problems that are problematic for quantum simulation. One technology of particular interest is the multi-mode superconducting resonator capable of storing multiple qubits in one device. We observe that these cavities have a natural virtual topology that aligns particularly well with quantum simulation problems, and exhibit much longer lifespans in comparison to other planar superconducting hardware. In this paper we present MUCIC, we discuss the simple integration of these devices into the current landscape and their implications to quantum simulation, motivated by their alignment to the quantum simulation problem, and potential as a quantum memory candidate. We report the development of MUCICs transpiler, leading to reductions of up to 82% in quantum simulation circuit depths. Additionally, our investigation demonstrates improvements of up to 19.4% in converged results from Variational Quantum Algorithms.

==> texts/discussion.tex <==
\section{Discussion}


==> texts/texts_old/background.tex <==
\section{Background}
\subsection{Quantum Computing}

Gate-based quantum computing is a computational paradigm that relies on quantum gates to manipulate qubits and perform computation. In contrast to classical computing, where a bit can only take on a value of 0 or 1, qubits can exist in a linear superposition of both $|0\rangle$ and $1\rangle$, represented by the vectors $|0\rangle = [1,0]^T$ and $|1\rangle = [0,1]^T$. This enables quantum computers to perform certain types of computations much faster than classical computers.

Quantum gates are the building blocks of gate-based quantum computing. These gates are similar to classical logic gates, but they operate on qubits and have restrictions such as each gate must be unitary and hermitian, due to the laws of quantum mechanics. Examples of commonly used quantum gates include the Hadamard gate, which can transform a ground state qubit ($|0\rangle$) into an equal superposition of the 0 and 1 states ($\frac{1}{\sqrt{2}}(|0\rangle+|1\rangle)$), and the CNOT gate, which can entangle two qubits.

To perform computations in gate-based quantum computing, a series of gates must be applied to a set of qubits in a particular sequence. The sequence of gates applied determines the outcome of the computation. However, one of the main challenges in gate-based quantum computing is decoherence, which occurs when qubits interact with their environment and their information decays. This can lead to errors in the computation, making it difficult to reliably perform complex calculations.

To address the issue of decoherence, researchers have developed quantum error correction and mitigation techniques, which aim to mitigate the issue of decoherence and gate errors. These techniques involve techniques such as encoding information in a larger hilbert space \cite{barends2014superconducting}, allowing for the detection and correction of errors, or by applying techniques such as Dynamical Decoupling \cite{viola1999dynamical}. However, techniques such as error correction can be challenging, as it requires significant resources.

Gate-based quantum computing is a promising approach to solving problems that are beyond the capabilities of classical computers. There are still many challenges to be addressed, ongoing research in this field holds the potential to revolutionize industries such as cryptography, chemistry, and optimization.

\subsection{Heterogenous Quantum Computing}

Presently, homogeneous monolithic quantum computers serve as the cornerstone of quantum computing technology, exemplified by cutting-edge devices such as the superconducting 433-qubit IBM-Q Osprey and the 22-qubit trapped ion Aria system. Each of these devices inherit their architectural problems, such as superconducting transmons being susceptible to decoherence due to substrate loss \cite{devoret2004superconducting}, and trapped ion quantum computers being extremely challenging to scale \cite{bruzewicz2019trapped}.

Approaches to hetereogenous quantum computing have come up in recent years, with proposals such as ARQUIN \cite{ang2022architectures}. Within ARQUIN exists an architecture for distributed quantum computing by coupling superconducting qubits on the edge of quantum processors with an optical link through the use of Microwave-to-Optical transduction. This coupling overcomes the short-range coupling nature of superconducting qubits, however at what proves to be an exceptionally high cost. Similar technologies within one device has also been proposed, where amazon proposed the use of CAT-qubits with Transmons in an error correcting code \cite{Hann2023MM}. Both of these are superconducting technologies, however display different computational properties.

Recent works of particular interest is the cavity-transmon coupled system, which have been demonstrated to have T1 times of up to a staggering \textbf{$34ms$}. Not only do cavities offer substantial resilience to decoherence, one cavity can be engineered to store multiple qubits using multiple resonance modes, with up to 9 modes being experimentally demonstrated \cite{chakram2021seamless}, with efficient cavity-transmon coupling allowing for information to be swapped in and out of the cavity \cite{milul2023superconducting,teoh2022dual}. HetArch[HetArch Citation] motivates the use of a cavity as a memory, and transmons as compute, laying out the heterogenous architecture building blocks for future devices, demonstrating substantial advantages over quantum primitives such as Entanglement Distillation, Code Teleportation, and Error Correction.  


\subsection{Variational Quantum Eigensolver}
The Variational Quantum Eigensolver (VQE) \cite{parrish+:prl19, li+:asplos22} is an innovative hybrid quantum-classical algorithm that aims to efficiently determine the lowest energy, or ground state, of molecular systems. This task is of significant importance for various fields, including chemistry, material science, and pharmaceutical research, as it allows researchers to predict the behavior of molecules and design novel materials with desired properties. The development of VQE has been driven by the growing interest in quantum computing and its potential to tackle problems that are intractable for classical computers.

VQE is designed for near-term, noisy intermediate-scale quantum (NISQ) devices, which are characterized by limited qubit numbers and high error rates. This hybrid algorithm combines the strengths of quantum and classical computing, exploiting the ability of quantum computers to handle large state spaces while leveraging classical optimization techniques to circumvent the limitations of NISQ devices .

To solve for the lowest energy state of a molecule, VQE employs a parameterized quantum circuit, also known as an ansatz, which approximates the ground state wavefunction based on the hamiltonian of the molecule. The Hamiltonian of the system can be represented as a linear combination of Pauli strings, where each Pauli string represents a term in the Hamiltonian. Then the ansatz is generated based on the Pauli strings. 

 \begin{figure}[htb]
    \centering
\includegraphics[width=0.45\textwidth]{figure/vqe_tree.pdf}
    \caption{Generate VQE ansatz using cavity} 
    \label{fig:VQE_ansatz}
\end{figure}

 VQE uses classical optimizers to iteratively adjust the parameters of the quantum circuit until the energy expectation value converges to a minimum. This hybrid approach allows VQE to leverage the advantages of both quantum and classical computing, providing a promising path to solving complex molecular problems on near-term quantum devices. We show the process in Figure. \ref{fig:VQE_ansatz}


\subsection{Quantum Approximate Optimization Algorith}
The Quantum Approximate Optimization Algorithm (QAOA) is a quantum algorithm proposed by Farhi et al\cite{Farhi2022}. in 2014 that aims to solve combinatorial optimization problems by using a quantum computer. QAOA has been studied extensively in recent years due to its potential for solving a wide range of optimization problems \cite{li+:asplos19} \cite{murali+:asplos19}\cite{siraichi+:oopsla19}\cite{siraichi+:cgo18}\cite{ tan+:iccad20}\cite{ sivarajah+:qst20}

The QAOA algorithm is based on a variational approach to optimization, in which the problem is mapped to a Hamiltonian, and the ground state of this Hamiltonian is found using a quantum computer. The Hamiltonian is constructed using a set of cost and driver Hamiltonians, which are parameterized by a set of angles $\boldsymbol{\gamma}$ and $\boldsymbol{\beta}$ respectively. The cost Hamiltonian encodes the objective function to be optimized, while the driver Hamiltonian prepares a superposition of states.

The QAOA algorithm can be written as follows:

\begin{enumerate}
\item Prepare an initial state $|s\rangle$, which is usually chosen to be a uniform superposition of all possible bit strings.
\item Apply the QAOA circuit, which consists of $p$ layers of cost and driver Hamiltonians, where each layer is defined as:
\begin{align*}
U(C,\gamma_j)&=e^{-i\gamma_j C}\\
U(B,\beta_j)&=e^{-i\beta_j B}
\end{align*}
where $C$ and $B$ are the cost and driver Hamiltonians, and $\gamma_j$ and $\beta_j$ are the angles at the $j^{th}$ layer.
\item Measure the final state in the computational basis to obtain a bit string that is an approximate solution to the optimization problem.
\end{enumerate}

The QAOA algorithm is optimized by finding the optimal values of the angles $\boldsymbol{\gamma}$ and $\boldsymbol{\beta}$ that minimize the cost function .
 The cost function is defined as the expectation value of the cost Hamiltonian $C$ with respect to the final state $|\psi\rangle$:

\begin{equation}
    C(\boldsymbol{\gamma},\boldsymbol{\beta})=\langle \psi(\boldsymbol{\gamma},\boldsymbol{\beta})|C|\psi(\boldsymbol{\gamma},\boldsymbol{\beta})\rangle
\end{equation}
    
 

where $|\psi(\boldsymbol{\gamma},\boldsymbol{\beta})\rangle$ is the final state obtained after applying the QAOA circuit.

QAOA has been shown to be effective in solving a variety of optimization problems, including Max-Cut, Max-3SAT, and graph partitioning\cite{lao+:isca22, alam+:dac20, alam+:micro20, li+:asplos22}\etal \cite{tan+:iccad20}. However, it is still an open question whether QAOA can outperform classical optimization algorithms in practice, and how many layers are needed to achieve good performance.

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=\textwidth]{figure/homog_vs_het.png}
    \caption{Comparison of current homogenous quantum computing architectures to future heterogenous architectures. \textbf{(a)} IBM Honeycomb represents 15 qubits coupled in a Honeycomb coupling map (IBM) comprised of superconducting qubits. \textbf{(b)} IonQ (Trapped Ion) represents a 5-qubit trapped ion homogen  ous architecture with native all-to-all connectivity. \textbf{(c)} Cavity-Transmon represents the proposed near term attainable architecture, comprised of two cavities coupled to two qubits, with each qubit having coupling. Each cavity is a mulit-mode cavity, allowing for the storage of multiple qubits per cavity, with relatively higher T1/T2 times compared to the transmons they are coupled to. Orange lines under Cavity-Transmon represent the SWAPping operation between Cavities and Transmons, and the black line between the transmons represents a Josephson junction coupling the two transmons.}
    \label{fig:homog_vs_het}
\end{figure*}


\subsection{Near Term Quantum Hardware}

\feicmd{here, I suggest add some near term challenges also ,which has high error rate, then tal about the benefit for heterogenous quantum computing, shift to the motivation of our paper and prepare a good start point for the method section}
Quantum computing has seen rapid development in recent years, with various technologies showing promise for implementing quantum bits (qubits) and operations. In this section, we will discuss the current technologies, their downsides, the benefits of combining different approaches, with a focus on cavities coupled with transmons, and the future of quantum hardware.

Several technologies have been proposed and implemented for quantum computing. Superconducting qubits, which are artificial atoms fabricated on a chip using superconducting materials, have relatively high coherence times and can be controlled using microwave pulses. Examples of superconducting qubits include transmons, Xmons, and flux qubits. Trapped ions represent another approach, where individual ions are trapped using electromagnetic fields and manipulated using lasers. This technology boasts high fidelity and long coherence times but faces challenges in scaling and control complexity.

Topological qubits are based on anyonic systems, with quantum information stored in the global topological properties of the system. These qubits offer intrinsic fault tolerance but are currently in the early stages of experimental realization. Photonic qubits utilize photons as carriers of quantum information, with operations performed using linear optical elements. Although they are robust against decoherence, scaling remains a challenge due to the probabilistic nature of photon-photon interactions. Lastly, quantum dots are semiconductor-based qubits where the quantum state is encoded in the electron's spin or charge. They offer the potential for high-speed operations but face challenges in coherence and fabrication.

Despite their unique advantages, each technology has its challenges. Superconducting qubits are susceptible to environmental noise, leading to a loss in coherence. Additionally, fabrication imperfections can result in variations in qubit properties. Trapped ions, while demonstrating high fidelity and long coherence times, face difficulties in scaling to a large number of qubits and performing parallel operations due to the need for precise control of individual ions.

Combining different technologies can potentially mitigate the limitations of each individual approach. A notable example is the integration of cavities coupled with transmon qubits. This hybrid approach takes advantage of the high coherence times and strong coupling strengths offered by superconducting qubits, while also leveraging the favorable properties of cavity-based systems. This combination can lead to improved error rates, better control, and increased flexibility in designing quantum architectures.

As research progresses, the future of quantum hardware is expected to see further development and refinement of existing technologies, as well as the emergence of new approaches. Heterogeneous architectures, which combine different technologies, are likely to play an important role in overcoming the limitations of individual systems. By leveraging the strengths of various technologies, such as cavities coupled with transmons, researchers can develop more robust, scalable, and efficient quantum computing platforms. Additionally, advances in error correction and fault-tolerant techniques will be crucial for the realization of large-scale, practical quantum computers.




==> texts/texts_old/conclusion.tex <==
\section{Conclusion}

==> texts/texts_old/introduction.tex <==
\section{Introduction}
Quantum computing has seen tremendous development in recent years motivated by its potential to solve complex problems that are intractable for classical computers. Quantum computers are theoretically able to perform certain calculations exponentially faster than classical computers. For example it can solve classical intractable  problems such as factoring \cite{shor:siam99}, chemistry simulation \cite{peruzzo+:naturecomm14,Kandala+:Nature17}, and large database search \cite{grover:astc96}. Although Quantum Computing can theoretically provide an advantage, there is an immense demand on both the hardware and software stack to produce usable results. To properly utilise the advantages quantum computing could provide, it is crucial to have developments not only improvements in hardware, such as the number of qubits and their coherence time, but also advancements in quantum algorithms and software to fully exploit the potential of quantum computing.

One Noisy Intermediate Scale Quantum (NISQ)  \cite{shor+:focs94, linke+:sa17, greenbaum+:arxiv15} era problems that have recieved a large amount of interest are Variational Quantum Algorithms. Optimization problems involve finding the best solution among a large number of possible solutions, and they have numerous applications in fields such as finance, logistics, and machine learning. Variational quantum algorithms (VQA) are well-suited for near-term quantum devices (NISQ) as they are designed to be noise-friendly, particularly to errors in physical gate implementation where the learnt parameters can compensate for the errors in implementation; however, they are not immune to non-Markovian or stochastic errors that can arise from the imperfect nature of quantum devices. 

The Quantum Approximate Optimization Algorithm (QAOA) \cite{farhi+:arxiv16,alam+:dac20}is a promising quantum optimization algorithm that has shown success in finding approximate solutions to combinatorial optimization problems such as MaxCut. While it is well-known that increasing the depth of QAOA circuits improves the expressibility of the circuit, physically realizing these circuits becomes challenging due to limited coherence times and gate errors. 

One exciting domain is quantum heterogeneous architectures, combining the benefits of multiple technologies into one quantum system. From coupling superconducting systems to optical links [ARQUIN], attaining long-distance entanglement over centimeter-scale chips in separate fridges, or coupling transmons to cavities and designing specifically laid out chiplets aimed at accomplishing quantum computing primitives [HETARCH]. The motivation to combine these technologies, is that each technology brings certain advantages over the other such as increased lifespans or connectivity. However, the cost of coupling technologies can be large, and often larger than the benefits gained by employing the coupling. An example of where different technologies are very useful is the magnitude higher T1 and T2 times of cavities in comparisons with superconducting qubits, whereby gate based computation on superconducting qubits is easier. 

With heterogenous architectures promising to provide large performance jumps in quantum computing in the future, We motivate application specific heterogenous quantum computing architectures in the near term, with hardware that is not too far out from todays engineering. We propose a dual-cavity-transmon system, alongside a scheduler for transmon-cavity data movement tailored to the QAOA algorithm. Our proposed architecture is an early look at the potential of heterogenous architectures, and how intelligent system design coupled with targeted technology coupling can provide substantial advantages to both the NISQ-era, pre-logical qubits, and beyond.

==> texts/texts_old/results.tex <==
\section{Results}

\subsection{Evaluating Cavity-Transmon Architecture}

We evaluate our Cavity-Transmon architecture via noisy simulation. We use Python 3.9.5, and Qiskit 0.43.0. Simulations are performed by applying T1/T2 decays according to idling times, and gate times. Gate times are set to 40ns for single qubit gates, 100 ns for CX gates, and 100 ns for SWAP-in or SWAP-out between cavities and transmons. Idling times are computed based on an as-soon-as-possible scheduler, and the set gate times. The basis gates set for superconducting qubits are the IBM-Q basis gates, $[CX,RZ(\theta),SX,X,Id]$. We evaluate the architecture on the VQE PROBLEMS GO HERE, and a set of MaxCut problem graphs. Each graph is evaluated with 4 experiment settings, ranging the number of layers based on the QAOA ansatz from 3 layers - 6 layers. The graph sizes represented are 4,6,8, and 10. 

\begin{figure*}
\scalebox{0.9}{
\Qcircuit @C=1.0em @R=0.2em @!R { \\
	 	\nghost{{compute}_{0} :  } & \lstick{{compute}_{0} :  } & \gate{\mathrm{R_Y}\,(\theta_1)} & \gate{\mathrm{R_Z}\,(\theta_2)} & \qswap & \gate{\mathrm{R_Y}\,(\theta_3)} & \gate{\mathrm{R_Z}\,(\theta_4)} & \qw & \ctrl{1} & \qswap & \qswap & \ctrl{1} & \qw & \qw & \ctrl{1} & \qswap & \qw \barrier[0em]{5} & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{compute}_{1} :  } & \lstick{{compute}_{1} :  } & \gate{\mathrm{R_Y}\,(\theta_5)} & \gate{\mathrm{R_Z}\,(\theta_6)} & \qw & \qswap & \gate{\mathrm{R_Y}\,(\theta_7)} & \gate{\mathrm{R_Z}\,(\theta_8)} & \targ & \qw & \qw & \targ & \qswap & \qswap & \targ & \qw & \qswap & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{cavity}_{0} :  } & \lstick{{cavity}_{0} :  } & \qw & \qw & \qswap \qwx[-2] & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qswap \qwx[-1] & \qw & \qw & \qswap \qwx[-1] & \qw & \meter & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{cavity}_{1} :  } & \lstick{{cavity}_{1} :  } & \qw & \qw & \qw & \qswap \qwx[-2] & \qw & \qw & \qw & \qw & \qswap \qwx[-3] & \qw & \qw & \qw & \qw & \qswap \qwx[-3] & \qw & \qw & \qw & \meter & \qw & \qw & \qw & \qw\\
	 	\nghost{{cavity}_{2} :  } & \lstick{{cavity}_{2} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qswap \qwx[-3] & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \meter & \qw & \qw & \qw\\
	 	\nghost{{cavity}_{3} :  } & \lstick{{cavity}_{3} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qswap \qwx[-5] & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \meter & \qw & \qw\\
	 	\nghost{\mathrm{{creg} :  }} & \lstick{\mathrm{{creg} :  }} & \lstick{/_{_{4}}} \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \dstick{_{_{\hspace{0.0em}0}}} \cw \ar @{<=} [-4,0] & \dstick{_{_{\hspace{0.0em}1}}} \cw \ar @{<=} [-3,0] & \dstick{_{_{\hspace{0.0em}2}}} \cw \ar @{<=} [-2,0] & \dstick{_{_{\hspace{0.0em}3}}} \cw \ar @{<=} [-1,0] & \cw & \cw\\}}
    \caption{Hardware Efficient Adaption of the Variational Quantum Eigensolver Ansatz for Dual-Cavity Dual-Transmon architecture based on Algorithm. \ref{alg:iterative_qubit_operation}, comprising 1 layer.  Cavity and transmons begin in the ground state, and SWAP's represent either SWAP-IN or SWAP-OUT operations. All SWAP operations are performed between a ground state qubit ($|0\rangle$), and an qubit actively part of the algorithm ($|\Psi\rangle$).}
    \label{fig:qaoa_circuit}
\end{figure*}

\subsection{VQE Evaluation}
\subsection{QAOA Evaluation}


\begin{figure*}
    \centering
    \scalebox{0.62}{
    \Qcircuit @C=1.0em @R=0.2em @!R { \\
	 	\nghost{{compute}_{0} :  } & \lstick{{compute}_{0} :  } & \gate{\mathrm{H}} & \qswap & \gate{\mathrm{H}} & \qw & \qswap & \qw & \qswap & \gate{\mathrm{R_X}\,(\mathrm{Beta})} & \qw & \qswap & \qw & \qswap & \gate{\mathrm{R_X}\,(\mathrm{Beta})} & \qw & \qswap & \qw & \qswap & \qw & \ctrl{1} & \qswap & \qw & \qswap & \qw & \ctrl{1} & \qswap & \qw \barrier[0em]{5} & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{compute}_{1} :  } & \lstick{{compute}_{1} :  } & \gate{\mathrm{H}} & \qw & \qswap & \gate{\mathrm{H}} & \qw & \qswap & \qw & \qswap & \gate{\mathrm{R_X}\,(\mathrm{Beta})} & \qw & \qswap & \qw & \qswap & \gate{\mathrm{R_X}\,(\mathrm{Beta})} & \qw & \qswap & \qw & \qswap & \gate{\mathrm{R_Z}\,(\mathrm{Gamma})} & \qw & \qswap & \qw & \qswap & \gate{\mathrm{R_Z}\,(\mathrm{Gamma})} & \qw & \qswap & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{cavity}_{0} :  } & \lstick{{cavity}_{0} :  } & \qw & \qswap \qwx[-2] & \qw & \qw & \qw & \qw & \qswap \qwx[-2] & \qw & \qw & \qswap \qwx[-2] & \qw & \qw & \qw & \qw & \qw & \qw & \qswap \qwx[-2] & \qw & \qw & \qswap \qwx[-2] & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \meter & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{cavity}_{1} :  } & \lstick{{cavity}_{1} :  } & \qw & \qw & \qswap \qwx[-2] & \qw & \qw & \qw & \qw & \qswap \qwx[-2] & \qw & \qw & \qswap \qwx[-2] & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qswap \qwx[-3] & \qw & \qw & \qswap \qwx[-3] & \qw & \qw & \qw & \meter & \qw & \qw & \qw & \qw\\
	 	\nghost{{cavity}_{2} :  } & \lstick{{cavity}_{2} :  } & \qw & \qw & \qw & \qw & \qswap \qwx[-4] & \qw & \qw & \qw & \qw & \qw & \qw & \qswap \qwx[-4] & \qw & \qw & \qswap \qwx[-4] & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \meter & \qw & \qw & \qw\\
	 	\nghost{{cavity}_{3} :  } & \lstick{{cavity}_{3} :  } & \qw & \qw & \qw & \qw & \qw & \qswap \qwx[-4] & \qw & \qw & \qw & \qw & \qw & \qw & \qswap \qwx[-4] & \qw & \qw & \qswap \qwx[-4] & \qw & \qswap \qwx[-4] & \qw & \qw & \qswap \qwx[-4] & \qw & \qswap \qwx[-4] & \qw & \qw & \qswap \qwx[-4] & \qw & \qw & \qw & \qw & \meter & \qw & \qw\\
	 	\nghost{\mathrm{{creg} :  }} & \lstick{\mathrm{{creg} :  }} & \lstick{/_{_{4}}} \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \dstick{_{_{\hspace{0.0em}0}}} \cw \ar @{<=} [-4,0] & \dstick{_{_{\hspace{0.0em}1}}} \cw \ar @{<=} [-3,0] & \dstick{_{_{\hspace{0.0em}2}}} \cw \ar @{<=} [-2,0] & \dstick{_{_{\hspace{0.0em}3}}} \cw \ar @{<=} [-1,0] & \cw & \cw\\}}
    \caption{Quantum Approximate Optimization Algorithm Ansatz Circuit Example Comprising two bimodal cavities (cavity), and two transmons (compute), with $n_{graph-nodes}=4$, and $p_{layers}=1$. Cavity and Transmon simulation settings are the same for QAOA and VQE.}
    \label{fig:qaoa_circuit}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{figure/qaoa_results.pdf}
    \caption{Analysis of QAOA results on 16 settings comparing homogenous transmon coupling with dual-cavity dual-transmon design. Transmon layout represents a Honeycomb lattice from IBM-Q, with the basis gate suite of ['cx','rz','x','sx','id']. Transmons in our design support the same set of basis gates, and Cavity-Transmon links support SWAP-IN and SWAP-OUT. }
    \label{fig:qaoa_results}
\end{figure*}

==> texts/texts_old/system.tex <==
\section{Methodology}


In this section, we investigate the limitations of NISQ-era hardware, and highlight the motivation for Heterogenous Architecture design for Variational Quantum Algorithms in the near term. We begin by discussing the current way we adopt variational quantum algorithms to homogeneous NISQ-era hardware, highlightin

\subsection{Variational Quantum Algorithms on Near Term Hardware}

Variational Quantum Algorithms (VQA), such as the Variational Quantum Eigensolver (VQE), Quantum Approximate Optimization Algorithm (QAOA), or Quantum Neural Networks (QML), are examples of noise-resilient algorithms in the near term. These algorithms accomplish this feat by utilizing parameterised gate operations such as $R_Y$ or $R_Z$ gates. This allows for over and under rotations to compensate for improper calibration of qubit gates. This highlights their resilience to parametric errors, however there exists a suite of other quantum error channels that can decohere a system. For example, the non-Markovian error channel of T1 and T2 decay are much more challenging to be captured by learnt rotations. Furthermore, many ansatz for these algorithms can place significant constraints on certain hardware's topology. On superconducting systems, such as IBM's Honeycomb architectures visualized in Figure \ref{fig:homog_vs_het}, the QAOA ansatz, or Chemistry-inspired VQE ansatz can lead to substantial topological cost via the use of CX gates to perform live-routing of qubits across the system. For trapped ion systems, although the connectivity is natively all-to-all, which reduces transpilation cost, however the scalability of trapped ion systems is challenged by the difficulty in scaling up trapped ion counts, as well as slower gate times. poses substantial challenges,
Therefore, although VQA's are noise-resillient, they are not noise-immune. They still exhibit limits on depth and width of quantum circuits that can solve certain VQA problems.

\subsection{Near Term Transmon-Cavity Coupled Architecture}

The computational demands on quantum computers to surmount the NISQ era are undoubtedly immense. The homogeneous computer architecture argument continues to exist in parallell, with questions such as \textbf{\textit{Will transmons end up being better than trapped ions?}} or \textbf{\textit{How large of a 2-D homogeneous superconducting system can we build in a single dilution refrigerator?}}, we continue to focus on systems without specific focus on quantum primitives, which form the foundation of many quantum computing algorithms. Recently demonstrated in HetArch[ToBeReleased], designing Heterogeneous chiplets comprising multiple technologies, specifically tailored to accomplishing quantum primatives can provide substantial computational advantage in primitives such as distilling high-fidelity EPR pairs, to code teleportation between different logical codes. HetArch argues for cavities to be used and referred to as a "Quantum Memory". These cavities are coupled with specifically laid out transmons, which perform the compute of the quantum routine. We use this future-heterogeneous architecture to motivate near-term attainable heterogeneous architecture that outperform our current homogeneous processors with application to, however not exclusive, Variational Quantum Algorithms.

Our architecture rests on engineering efforts works in cavities and their transmon coupling \cite{zhang2022drive}.  Demonstrated in Teoh. et. al. \cite{teoh2022dual}, a dual-transmon coupled cavity has been physically demonstrated. Furthermore, Chakram et. al. \cite{chakram2021seamless} demonstrates a 9-mode cavity with high T1/T2 lifespans. Finally, Milul et. al. \cite{milul2023superconducting} demonstrates a high-lifespan cavity with a T2 time of up to \textbf{$34ms$}. 

We propose a quantum processor comprising two superconducting qubits (\textbf{T-1,T-2}), and two multi-mode cavities (\textbf{C-1,C-2}). Each cavity can be represented by an $n$ mode register, where $n$ is the number of modes available the cavity.
The cavity begins in the state of $|Cavity\rangle_n = [|0\rangle_0,|0\rangle_1,...,|0\rangle_n]$. \textbf{T-1} is coupled to \textbf{T-2}. Qubits \textbf{T-1 \& T-2} are coupled to both cavities. No single gate operations are supported within each cavity, and the only operation that is supported between cavity and superconducting qubit is a SWAP-IN and SWAP-OUT, whereby a superconducting qubits state can be swapped in or out of the multiple cavity modes. The transmons support a computationally complete suite of basis gates. This architecture is outlined in Figure \ref{fig:homog_vs_het}. Orange lines describe the SWAP-IN SWAP-OUT functionality of the cavity, and black lines represent a coupling between qubits, supporting entangling operations (CX for transmon, Mølmer-Sørensen for the trapped ion).
\subsection{Example Cavity-Transmon System}
As a concrete example, we walk through an example of generating a 4-qubit GHZ state on the Cavity-Transmon architecture. The cavities are each 2-mode cavities respectively, and each mode begins in the ground state of $|0\rangle$, represented by the register of $|Cavity\rangle_0 = |Cavity\rangle_1 = [|0\rangle,|0\rangle]$. 
We begin by placing $T-1$ in an equal superposition of $|0\rangle$ and $|1\rangle$, state of $|T-1\rangle = \frac{1}{\sqrt{2}}(|0\rangle+|1\rangle)$. A CX is applied between $T-1$ and $T-2$, generating a 2-qubit GHZ state. Qubits $T-1$ is swapped into $Cavity-1$'s 0th index, resulting in $T-1$ being in the ground state of $|0\rangle$. $T-2$ is entangled with a CX with $T-1$, continuing the GHZ state generation chain, followed by $T-2$ swapped into $Cavity-2$. Finally, $T-1$ is entangled through a CX gate with $T-2$, and the qubits are transferred into the cavities. This results in the two cavities two modes being populated by a fully entangled GHZ state $|0000\rangle + |1111\rangle$). We depict this in Figure NNN.

\subsection{Hardware Efficient Scheduling}

VQA's commonly use hardware-efficient or domain-specific circuit structures, such as the linear-entanglement scheme or chemistry inspired ansatz based on the Jordan Wigner transformation. Domain specific ansatz lend better performance in their domain, however often have much higher circuit depth. Our solution efficiently transpiles these ansatz natively through, with the ability to sequentially walk through entanglement chains without topological constraints. As an example, for the hardware efficient ansatz, which is a linear entanglement scheme, we describe how one can perform this entangling scheme in Algorithm \ref{alg:iterative_qubit_operation}. This procedure chains CX gates between each qubit. If a root-CX chain from Hamiltonian Simulation is used, this follows the same procedure, however non-interacting qubits (I in the Pauli-string) do not need to be moved in or out of memory. For single qubit operations, a similar scheduler would perform single qubit operations instead of entangling operations, and can perform data movement in parallel instead of the sequential nature of entangling schemes.

\begin{algorithm}
\caption{Hardware Efficient Ansatz Scheduling for Entangling}
\label{alg:iterative_qubit_operation}
\begin{algorithmic}[1]
\REQUIRE $Q_1, Q_2$ sequence of qubits;
\REQUIRE $Cavity-1, Cavity-2$ Memory cavities of mode N;
\REQUIRE $CX$: quantum operation to apply on qubit pairs
\STATE Prepare $Q_1$ into initial state
\FOR{$i = 1$ to $(n)//2 + nMod2$}
    \STATE $CX$(Q_1,Q_2)
    \STATE Move $Q_1$ into Cavity-1 
    \STATE Move $Cavity-1_i$ into Q-1
    \STATE $CX$(Q_1,Q_2).
    \STATE Move $Q_2$ into Cavity-2
    \STATE Move $Cavity-2_i$ into Q-2
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{Simulating Cavity-Transmon Architectures}

Unlike trapped ion or superconducting quantum processors which have commercially available hardware for experimental demonstration, cavity-transmon systems are not available. Therefore, we evaluate our architecture over noisy simulation. To simulate our architecture, we use a respective T1/T2 time on cavities of 1ms, the current demonstrated T1/T2 times for multi-mode cavities. We set a T1/T2 time of 0.1ms for transmons. We focus our comparison on comparing the cavity transmon architecture against monolithic homogeneous transmon design, laid out in a Honeycomb fashion depicted in Figure \ref{fig:homog_vs_het}. 
